Estimating Image Depth in the Comics Domain

Estimating the depth of comics images is challenging as such images a) are monocular; b) lack ground-truth depth annotations; c) differ across different artistic styles; d) are sparse and noisy. We thus, use an off-the-shelf unsupervised image to image translation method to translate the comics images to natural ones and then use an attention-guided monocular depth estimator to predict their depth. This lets us leverage the depth annotations of existing natural images to train the depth estimator. Furthermore, our model learns to distinguish between text and images in the comics panels to reduce text-based artefacts in the depth estimates. Our method consistently outperforms the existing state-ofthe-art approaches across all metrics on both the DCM and eBDtheque images. Finally, we introduce a dataset to evaluate depth prediction on comics. Our project website can be accessed at https://github.com/IVRL/ComicsDepth.

==> images/fig2.tex <==
\begin{figure}[hbt!]
\centering
\renewcommand{\thesubfigure}{}
\subfigure[Comics Input]
\centering
{\includegraphics[ width=0.4\linewidth]{images/input-fig2.png}}\hfill
\vspace{-11.5pt}
\subfigure[Predicted Depth]
\centering
{\includegraphics[width=0.4\linewidth]{images/input-depth-fig2.png}}\hfill
\vspace{-11.5pt}
\subfigure[Translated Image ]
\centering
{\includegraphics[width=0.4\linewidth]{images/translated-fig2.png}}\hfill
\vspace{-11.5pt}
\subfigure[Predicted Depth]
\centering
{\includegraphics[width=0.4\linewidth]{images/tranalated-depth-fig2.png}}\hfill
\vspace{-11.3 pt}
\caption{{Existing unsupervised monocular depth estimation models fail to predict the depth of images in the comics domain. We thereby, translate the } 
}\label{fig:monocular-model-prediction}\vspace{-10pt}
\end{figure}

==> images/teaser.tex <==
\begin{center}
\centering
\includegraphics[height=6.5cm, width =9.3cm]{images/Abstract.png}
\includegraphics[height=6.5cm, width =8.0cm]{images/teaser-2.png}
\captionof{figure}{\textbf{\Romannum{1}$)$} Estimating depth in the comics domain is subject to many \textbf{challenges}, including a) occlusions between characters; b) unusual object sizes (the bird here); c) unusual perspective; d) and e) different illustrative styles. \textbf{\Romannum{2}$)$} \textbf{Overview of our model}, which  uses an unsupervised I2I translation method to translate the comics image to the natural image domain and then, employs a contextual depth estimator with Laplacian edges and a feature-based GAN to ultimately predict depth. \textbf{\Romannum{3}$)$} Comparative depth estimation \textbf{results} using MIDAS~\cite{midas}, Contextual Depth Estimation (CDE)~\cite{CDE} and Ours. \textbf{\Romannum{4}$)$} \textbf{Application of our method} to image retargeting, where our depth estimation model guides the retargetting model~\cite{seam-carving}.}
\label{fig:teaser}
\end{center}
